Cross Space and Time: A Spatio-Temporal Unitized Model for Traffic Flow Forecasting

Predicting spatio-temporal traffic flow presents significant challenges due to complex interactions between spatial and temporal factors. Existing approaches often address these dimensions in isolation, neglecting their critical interdependencies. In this paper, we introduce the Spatio-Temporal Unitized Model (STUM), a unified framework designed to capture both spatial and temporal dependencies while addressing spatio-temporal heterogeneity through techniques such as distribution alignment and feature fusion. It also ensures both predictive accuracy and computational efficiency. Central to STUM is the Adaptive Spatio-temporal Unitized Cell (ASTUC), which utilizes low-rank matrices to seamlessly store, update, and interact with space, time, as well as their correlations. Our framework is also modular, allowing it to integrate with various spatio-temporal graph neural networks through components such as backbone models, feature extractors, residual fusion blocks, and predictive modules to collectively enhance forecasting outcomes. Experimental results across multiple real-world datasets demonstrate that STUM consistently improves prediction performance with minimal computational cost. These findings are further supported by hyperparameter optimization, pre-training analysis, and result visualization. We provide our source code for reproducibility at https://anonymous.4open.science/r/STUM-E4F0.

==> Table/datasets.tex <==
%D2STGCNN、STFGNN、STAE均有该表但不太一致，我以STFGNN为主了
\begin{table*}[ht]
\centering
%\setlength{\tabcolsep}{1.2mm}{}
\caption{Statistics and description of datasets we used.}
\begin{tabular}{c|cccccc}
\toprule
Dataset & \#Nodes & \#Edges & \#Frames & Time Range & Type\\ 
\hline
METR-LA & 207 & 1515 & 34,272 & 03/01/2012 – 06/27/2012 & Traffic speed\\
PEMS-BAY & 325 & 2369 & 52,116 & 01/01/2017 – 06/30/2017 & Traffic speed\\
PEMS03 & 358 & 547 & 26208 & 09/01/2018 – 11/30/2018 & Traffic flow\\
PEMS04 & 307 & 340 & 16992 & 01/01/2018 – 02/28/2018 & Traffic flow\\
PEMS07 & 883 & 866 & 28224 & 05/01/2017 – 08/06/2017 & Traffic flow\\
PEMS08 & 170 & 295 & 17856 & 07/01/2016 – 08/31/2016 & Traffic flow\\
\bottomrule
\end{tabular}
\label{tab:dataset}
\end{table*}


==> Table/different_dataset_performance.tex <==

% % table3:The improvement of one model in different datasets. STGCN is taken as a reference here.

% \begin{table*}[htbp!]
% %    \vspace{-6mm}
%   \centering
%   \setlength{\tabcolsep}{0.3mm}{}
%   \caption{The improvement of one model in different datasets. STGCN is taken as a reference here.}
%   \scalebox{0.85}{
%     \begin{tabular}{c|c|ccc|ccc}
%     \toprule
%     \multirow{2}[4]{*}{Datasets} & \multirow{2}[4]{*}{Model} & \multicolumn{3}{c|}{60min} & \multicolumn{3}{c}{Average} \\
%     \cmidrule{3-8}
%     &   & MAE~$\downarrow$   & RMSE~$\downarrow$ & MAPE~$\downarrow$ & MAE~$\downarrow$   & RMSE~$\downarrow$  & MAPE~$\downarrow$ \\ 
%     \midrule
%     \multirow{3}[2]{*}{PEMS04} & STGCN & 22.34 & 34.89 & 15.87\% & 20.67 & 32.29 & 14.86\% \\
%       & STGCN+ & 22.07 & 34.47 & 15.42\% & 20.37 & 31.94 & 14.36\% \\
%       \rowcolor{green!20} \cellcolor{white!20} & $\Delta$ & -0.27 & -0.43 & -0.45\% & -0.30 & -0.35 & -0.50\% \\
%     \midrule
%     \multirow{3}[2]{*}{PEMS08} & STGCN & 18.23 & 28.29 & 12.41\% & 16.65 & 25.64 & 11.55\% \\
%           & STGCN+ & 17.83 & 27.85 & 12.06\% & 16.38 & 25.42 & 11.18\% \\
%           \rowcolor{green!20} \cellcolor{white!20} & $\Delta$ & -0.40 & -0.44 & -0.35\% & -0.27 & -0.22 & -0.37\% \\
%     \midrule
%     \multirow{3}[2]{*}{PEMS03} & STGCN & 19.29 & 32.09 & 20.12\% & 17.17 & 28.68 & 18.38\% \\
%           & STGCN+ & 18.84 & 31.74 & 18.87\% & 16.85 & 28.33 & 17.50\% \\
%           \rowcolor{green!20} \cellcolor{white!20} & $\Delta$ & -0.45 & -0.35 & -1.25\% & -0.32 & -0.35 & -0.88\% \\
%     \midrule
%     \multirow{3}[2]{*}{PEMS07} & STGCN & 27.09 & 41.85 & 12.21\% & 24.26 & 37.33 & 11.14\% \\
%           & STGCN+ & 26.50 & 41.26 & 11.89\% & 23.90 & 36.96 & 10.94\% \\
%           \rowcolor{green!20} \cellcolor{white!20} & $\Delta$ & -0.59 & -0.59 & -0.32\%    & -0.37 & -0.36 & -0.20\% \\
%     \midrule
%     \multirow{3}[2]{*}{METR-LA} & STGCN & 3.58  & 7.47  & 10.46\% & 3.13  & 6.29  & 8.68\% \\
%           & STGCN+ & 3.54  & 7.43  & 10.40\% & 3.10  & 6.26  & 8.63\% \\
%           \rowcolor{green!20} \cellcolor{white!20} & $\Delta$ & -0.04 & -0.04 & -0.06\% & -0.03 & -0.04 & -0.05\% \\
%     \midrule
%     \multirow{3}[2]{*}{PEMSBAY} & STGCN & 2.04  & 4.61  & 4.81\% & 1.68  & 3.66  & 3.83\% \\
%           & STGCN+ & 1.99  & 4.53  & 4.73\% & 1.64  & 3.59  & 3.74\% \\
%           \rowcolor{green!20} \cellcolor{white!20} & $\Delta$  & -0.05 & -0.08 & -0.08\% & -0.04 & -0.06 & -0.09\% \\
%     \bottomrule
%     \end{tabular}
% }
%   \label{tab:different_dataset}%
% \end{table*}%

\begin{table}[htbp!]
  \centering
  \setlength{\tabcolsep}{0.45mm}{}
  \caption{The improvement of one model in all of six datasets.}
  \scalebox{0.9}{
    \begin{tabular}{c|ccc|ccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[4]{*}{dataset}} & \multicolumn{3}{c|}{60min} & \multicolumn{3}{c}{Average} \\
\cmidrule{2-7}         & MAE   & RMSE  & MAPE  & MAE   & RMSE  & MAPE \\
    \midrule
    \rowcolor{green!20} \cellcolor{white!20}PEMS04 & -0.84 & -0.95 & -0.62\% & -0.54 & -0.64 & -0.15\% \\
    \midrule
    \rowcolor{green!20} \cellcolor{white!20}PEMS08 & -0.49 & -0.40 & -1.05\% & -0.29 & -0.22 & -1.21\% \\
    \midrule
    \rowcolor{green!20} \cellcolor{white!20}PEMS03 & -0.45 & -0.35 & -1.25\% & -0.32 & -0.35 & -0.88\% \\
    \midrule
    \rowcolor{green!20} \cellcolor{white!20}PEMS07 & -0.59 & -0.59 & -0.32\% & -0.37 & -0.36 & -0.20\% \\
    \midrule
    \rowcolor{green!20} \cellcolor{white!20}METR-LA & -0.04 & -0.04 & -0.06\% & -0.03 & -0.04 & -0.05\% \\
    \midrule
    \rowcolor{green!20} \cellcolor{white!20}PEMSBAY & -0.05 & -0.08 & -0.08\% & -0.04 & -0.06 & -0.09\% \\
    \bottomrule
    \end{tabular}%
}
\vspace{-6mm}
  \label{tab:different_dataset}%
\end{table}%


==> Table/different_model_performance.tex <==

% Table2: The improvement of different models for one dataset. PEMS04 is taken as the reference dataset. And we have chosen STGCN, GWNet, AGCRN and LSTM as representatives by type of deep network.

\begin{table*}[t!]
  \centering
   \setlength{\tabcolsep}{2.0mm}{}
\caption{The improvement of different models in the PEMS04 dataset. Here, lower values indicate better performance. All six baselines have achieved significant improvements, denoted by $\Delta$.}
   \vspace{0.1mm}
   \scalebox{0.85}{
    \begin{tabular}{c|ccc|ccc}
    \toprule
    \multirow{2}[4]{*}{Model} & \multicolumn{3}{c|}{60min} & \multicolumn{3}{c}{Average} \\
    \cmidrule{2-7}
    & MAE$~\downarrow$   & RMSE$~\downarrow$  & MAPE$~\downarrow$ & MAE$~\downarrow$   & RMSE$~\downarrow$  & MAPE$~\downarrow$ \\
    \midrule
    HI    & 42.37 & 61.67 & 29.96 & 42.36 & 61.66 & 29.92\% \\
    VAR   & 26.76 & 40.28 & 20.94 & 23.51 & 36.39 & 17.85\% \\
    SVR   & 37.86 & 56.01 & 26.72 & 28.66 & 44.59 & 19.15\% \\
    \midrule
    LSTM  & 26.93 & 41.95 & 18.34\% & 22.57 & 35.52 & 15.20\% \\
    LSTM+ & 26.34 & 41.30 & 18.26\% & 22.18 & 35.16 & 15.08\% \\
    \rowcolor{green!20} \cellcolor{white!20} $\Delta$ & -0.59 & -0.64 & -0.08\% & -0.39 & -0.37 & -0.12\% \\
    \midrule
    STGCN & 22.34 & 34.89 & 15.87\% & 20.67 & 32.29 & 14.86\% \\
    STGCN+ & 22.07 & 34.47 & 15.42\% & 20.37 & 31.94 & 14.36\% \\
    \rowcolor{green!20} \cellcolor{white!20} $\Delta$ &-0.27 & -0.43 & -0.45\% & -0.30 & -0.35 & -0.50\% \\
    \midrule
    GWNet & 23.07 & 35.35 & 17.34\% & 20.43 & 31.93 & 14.62\% \\
    GWNet+ & 20.89 & 32.96 & 14.92\% & 19.22 & 30.62 & 13.54\% \\
    \rowcolor{green!20} \cellcolor{white!20} $\Delta$  & -2.18 & -2.39 & -2.42\% & -1.21 & -1.31 & -1.08\% \\
    \midrule
    AGCRN & 20.41 & 32.87 & 14.38\% & 19.10 & 30.80 & 13.40\% \\
    AGCRN+ & 19.97 & 32.37 & 13.78\% & 18.81 & 30.51 & 13.05\% \\
    \rowcolor{green!20} \cellcolor{white!20} $\Delta$  & -0.44 & -0.50 & -0.60\% & -0.29 & -0.29 & -0.35\% \\
    \midrule
    STAE  & 21.06 & 33.37 & 15.55\% & 19.31 & 30.86 & 13.85\% \\
    STAE+ & 20.40 & 32.38 & 15.00\% & 18.89 & 30.22 & 13.58\% \\
    \rowcolor{green!20} \cellcolor{white!20} $\Delta$   & -0.66 & -0.99 & -0.55\% & -0.42 & -0.64 & -0.27\% \\
    \midrule
    D2STGNN & 23.34 & 35.89 & 17.39\% & 20.75 & 32.36 & 15.91\% \\
    D2STGNN+ & 21.73 & 33.73 & 17.00\% & 19.73 & 31.05 & 14.86\% \\
    \rowcolor{green!20} \cellcolor{white!20} $\Delta$ & -1.61 & -2.16 & -0.39\% & -1.02 & -1.31 & -1.05\% \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:different_model}
\end{table*}
